The mass-loss, expansion velocities and dust production rates of carbon stars in the Magellanic Clouds

The properties of carbon stars in the Magellanic Clouds (MCs) and their total dust production rates are predicted by fitting their spectral energy distributions (SED) over pre-computed grids of spectra reprocessed by dust. The grids are calculated as a function of the stellar parameters by consistently following the growth for several dust species in their circumstellar envelopes, coupled with a stationary wind. Dust radiative transfer is computed taking as input the results of the dust growth calculations. The optical constants for amorphous carbon are selected in order to reproduce different observations in the infrared and optical bands of \textit{Gaia} Data Release 2. We find a tail of extreme mass-losing carbon stars in the Large Magellanic Cloud (LMC) with low gas-to-dust ratios that is not present in the Small Magellanic Cloud (SMC). Typical gas-to-dust ratios are around $700$ for the extreme stars, but they can be down to $\sim160$--$200$ and $\sim100$ for a few sources in the SMC and in the LMC, respectively. The total dust production rate for the carbon star population is $\sim 1.77\pm 0.45\times10^{-5}$~M$_\odot$~yr$^{-1}$, for the LMC, and $\sim 2.52\pm 0.96 \times 10^{-6}$~M$_\odot$~yr$^{-1}$, for the SMC. The extreme carbon stars observed with the Atacama Large Millimeter Array and their wind speed are studied in detail. For the most dust-obscured star in this sample the estimated mass-loss rate is $\sim 6.3 \times 10^{-5}$~M$_\odot$~yr$^{-1}$. The grids of spectra are available at: https://ambrananni085.wixsite.com/ambrananni/online-data-1 and included in the SED-fitting python package for fitting evolved stars https://github.com/s-goldman/Dusty-Evolved-Star-Kit .

==> emulateMNRAS.tex <==
\newcommand{\realfigure}[3]{
              \begin{figure}
              \includegraphics[width=84mm]{#1}
              %\includegraphics[width=84mm]{PSFILES/dummy.ps}
              \caption{#2}
              \label{#3}
              \end{figure}}

\newcommand{\realfiguretwo}[4]{
              \begin{figure*}
              \centering
	          \includegraphics[width=84mm]{#1}\hfill
	          \includegraphics[width=84mm]{#2}
              \caption{#3}\label{#4}
              \end{figure*}}
              


\newcommand{\mytab}[6]{
\begin{table}
\caption{#4}
\label{#5}
\begin{center}
\begin{#6}
\begin{tabular}{#1}
\hline 
#2
\hline
#3
\hline
\end{tabular}
\end{#6}
\end{center}
\end{table}
}

\newcommand{\mytabbig}[6]{
\begin{table*}
\begin{minipage}{126mm} 
\caption{#4}
\label{#5}
\begin{center}
\begin{#6}
\begin{tabular}{#1}
\hline 
#2
\hline
#3
\hline
\end{tabular}
\end{#6}
\end{center}
\end{minipage}
\end{table*}
}

